Systematic Mapping Study of Template-based Code Generation

Template-based code generation (TBCG) is a synthesis technique that produces code from high-level specifications, called templates. TBCG is a popular technique in model-driven engineering (MDE) given that they both emphasize abstraction and automation. Given the diversity of tools and approaches, it is necessary to classify existing TBCG techniques to better guide developers in their choices. The goal of this article is to better understand the characteristics of TBCG techniques and associated tools, identify research trends, and assess the importance of the role of MDE in this code synthesis approach. We conducted a systematic mapping study of the literature to paint an interesting picture about the trends and uses of TBCG. Our study shows that the community has been diversely using TBCG over the past 15 years. TBCG has greatly benefited from MDE. It has favored a template style that is output-based and high level modeling languages as input. TBCG is mainly used to generate source code and has been applied in a variety of domains. Furthermore, both MDE and non-MDE tools are becoming effective development resources in industry.

==> context.tex <==
\section{Two Modernization Projects} \label{sec:context}

In this section, we present the two projects where Fresche Legacy applied MDE.
The purpose of this section is to understand the complexity of this tedious modernization task.

\subsection{Synon modernization project}\label{sec:synon}

Fresche Legacy decided to make a first proof of concept for using MDE to automatically migrate a legacy application developed with Synon to a Java-based web application.
This project was chosen because Synon is already at a level of abstraction higher than RPG and therefore assumed that the complexity of the task will be lesser.
Synon dates from 1984 and is used to specify data and processes to be generated for AS/400 systems.
It is highly structured, with specifications for \Code{Files} (or database tables) as representations of the application data structures, \Code{Functions} to contain and organize the business logic, \Code{Action Diagram Elements} that correspond to the business logic where each element corresponds to a statement, \Code{Screens} to display representations, and \Code{Reports} for static data representations.
Synon can also be viewed as an early day modeling approach, being the precursor of Architected Rapid Application Development (ARAD) \cite{Gupta2003ARAD}, and even more general Computer Assisted Software Engineering (CASE) approaches.
One major advantage of starting the modernization process with Synon is that it provides a higher level of abstraction than the generated code and has many OO abstractions that are compatible with a modern modeling views of systems.

\subsubsection{Applying MDE}

\begin{figure}[htb]
	\centering
	\includegraphics[width=\linewidth, page=1]{images/workflow.pdf}
	\caption{Overview of the process to migrate Synon code to a web application}
	\label{fig:workflowSynon}
\end{figure}
%
\Fig{fig:workflowSynon} depicts the process of modernizing Synon applications using MDE.
First, they reverse engineer Synon code using MoDisco~\cite{Brunelière20141012} to extract the required information from the Synon repository and produce an Ecore model of the Synon code.
MoDisco also derived a metamodel for Synon.
The derived metamodel consists of 245 classes total (see \Table{tab:metamodel}).
Note that it also inherits from the Generic Abstract Syntax Tree Metamodel (GASTM) provided by MoDisco.
The extracted model is a 17.5 MB XMI file, containing the representation of 126 \Code{Files}, 263 \Code{Functions}, $13\,841$ \Code{Action Diagram Elements}, 32 \Code{Screens} and 25 \Code{Reports}.
%
\begin{table}[h]
\centering
\begin{tabular}{lcc}
	\toprule
	\textbf{Metamodel} & \textbf{Synon} & \textbf{RPG}	\\
	\midrule
	Number of classes    & 245   & 477 \\
	Number of references & 239   & 322 \\
	Number of attributes & 392   & 151 \\
	\bottomrule
\end{tabular}
\caption{Size of Synon and RPG metamodels}
\label{tab:metamodel}
\end{table}

With the use of Acceleo templates~\cite{Acceleo2016}, they generate a web-based implementation of the system from the Synon model.
\Table{tab:synon} summarizes the characteristics of the resulting generated application.
Most of the work implementing the templates is dedicated to the business logic and interaction with the database, implemented in Java.
The remaining generated artifacts are for the web front and configuration.
Note that this generation process ignored the \Code{Report} elements.
Up to 10\% of the lines of code in each file are comments.
%
\begin{table}[h]
\centering
\begin{tabular}{lrr}
	\toprule
	\textbf{Language} & \textbf{Files} & \textbf{Lines of code}  \\
	\midrule
	Java         & 1\,125 & 60\,396 \\
	CSS          & 2      & 18\,223 \\
	Javascript   & 101    & 9\,877  \\
	HTML         & 46     & 4\,347  \\
	LESS         & 19     & 3\,861  \\
	Maven        & 2      & 1\,274  \\
	JSON         & 6      & 174     \\
	XML          & 4      & 173     \\
	DOS Batch    & 1      & 127     \\
	Bourne Shell & 2      & 114     \\
	\midrule
	Total        & 1\,308 & 98\,566 \\
	\bottomrule
\end{tabular}
\caption{Characteristics of the generated application from Synon}
\label{tab:synon}
\end{table}

\subsubsection{Successful adoption}\label{sec:success}

The MDE-based Synon modernization project lasted one year, starting in September 2014.
The work was performed by one architect who, within that period of time, learned about MDE and the necessary tools.
He applied this acquired knowledge to design, implement, and test the project.
In the final month, five additional developers joined the project.
Their task was to create the templates for the code generator as well as the data to test the generated application.
%as the customer did not  provide Fresche Legacy with a complete set of data.
Once all the components of the process were completed, the migration from Synon to the Java code for this specific project took less than a day.

This pilot project was a success. 
Therefore the metamodel, reverse engineering tool, and templates are now being used in the core development of the company.
This MDE technique has been applied on three other projects.
Two of them are of similar scale as this one, in the order $10^5$ lines of code with around $10^3$ files produced.
From past experiences, projects of this scale required around 5 man-months effort to produce the final application manually.
With MDE, the two projects took around $1.5$ man-weeks to automatically produce the final application.
This represents a 20 times improvement in terms of time productivity for the developers.
This is considered a small scale project.
A medium size modernization project is typically in the order of $10^6$ lines of code with around $10^4$ files produced.
Medium projects require 69 man-years efforts.
Recently, Fresche Legacy estimated a Synon modernization project of this using MDE size to $1.8$ man-years.



%For comparison, a handwritten modernization process from Report Program Generator (RPG) \cite{IMB1994RPGRef, IMB1994RPGUG, yaeger1995programming} to Java, of equivalent size is characterized in Table \ref{tab:rpg}.\es{we need to discuss that}
%For the Synon generator there is still work to do. Among this work, there is the automatic conversion of Report Program Generator (RPG) and Cobol calls by the Synon application, reports and some other functionalities.


\subsection{RPG modernization project}\label{sec:rpg}

\begin{figure*}
	\centering
	\includegraphics[scale=.50, page=2]{images/workflow.pdf}
	\caption{Workflow of RPG to Java modernization}
	\label{fig:workflowRPG}
\end{figure*}
%
Currenly Fresche Legacy is developing the process of modernizing RPG applications to Java using MDE.
RPG is a language used to develop programs for AS/400 systems, released in 1959.
The language has significantly evolved since then.
Originally a procedural language with strong static typing, it used a fixed columns and line length so it could be input into the system with punch cards.
The current version used is RPG IV and allows for free format.
Many other functionalities were included to adapt the language to more modern requirements.
This raises a problem when modernizing legacy systems in RPG as there is no one pattern of design to follow.
The code can be structured to take advantage of reuse or to be delivered with punch cards, it may have access to a database, or be designed for sequential data, such as tapes.

\subsubsection{Scope prior to collaboration}

After a successful proof of concept with Synon, the company proceeded with migrating RPG-based projects.
Although there are similarities in how the code is generated, RPG being the source is a much more challenging endeavor than with Synon.
The major difficulty is the low level of abstraction of the legacy paradigm that needs to be migrated to an object-oriented paradigm.
Prior to automating the process with MDE, manual modernization projects produced a target application that relied on frameworks and libraries that emulate the behavior of the legacy application, only in a modern system.
Following the approach for Synon, an RPG model is extracted from the RPG code base and Acceleo templates are used to generate the target application.
In this case, the RPG metamodel was hand-written as a refinement of Generic Abstract Syntax Tree Metamodel (GASTM) (a sub section of Abstract Syntax Tree Metamodel specification \cite{ASTM201}), since MoDisco does not support RPG.
Furthermore, they implemented a parser that extract RPG code and produces an RPG model that conforms to the RPG metamodel.
The parser interfaces with MoDisco code in order to manipulate GASTM elements.
In this project, the resulting RPG model is a 16 MB XMI file, containing 145\,208 elements.
\Table{tab:metamodel} summarizes the characteristics of the RPG metamodel.
The process, illustrated on the top of \Fig{fig:workflowRPG}, is the scope of the project prior to our collaboration.

\subsubsection{Scope of the collaboration}

The collaboration of Fresche Legacy with us (the first two authors) aimed at providing a clear abstraction from the legacy system and its logic.
Prior to that, the resulting modernized application needed to be re-engineered in order to take advantage of optimizations of the new paradigm, whether it is for applications generated with the MDE approach or hand-coded.
This is also where clients change requests are implemented.
However, all the refactorings and optimizations performed at the code level are time consuming and error prone.
Therefore, we proposed to define a domain-specific language (DSL) that abstracts RPG details and emphasizes on the business logic of the application.
An ATL transformation produces a domains-specific model (DSM) conforming to this DSL from the RPG model.
Manual refactorings and optimizations are performed on the DSM before Acceleo templates generate the target application.
This process is illustrated in the box at the bottom of \Fig{fig:workflowRPG}.


%Apart from the inherent challenges of modernizing RPG applications, Fresche Legacy needed to automate the process using MDE
%to want to update the MDE workflow used, and start a collaboration with us. This issues start with creating an intermediate modeling language that provides a clear abstraction from the source system platform details, because current modernization relies on the use of emulation frameworks. This modeling language will also simplify any refactoring required on the system. This requirement is raised because there is knowlage on here to apply optimizations to the system one it is free from the original platform, but doing this refactoring at code level of such large code base is very time consuming and error prone, if done before de code generation it would benefit from the alleviation of that workload, and the refactoring patterns will be simpler to express at a business level. These refactorings alongside known optimizations also include cient requests, many times the trigger of the modernization process itself, such as integrating new technologies, for example mobile access.
%
%Nevertheless commercial compromises require de production of code as soon as possible, and because of the success and knowledge acquired during the proof of concept project, a code generation from RPG model to Java is also in development. This should provide results sooner than the intermediate DSL, and it is expected that most of the work producing the code generation templates can be mitigated, by reusing these template patterns on the DSL elements, because the essential information will be maintained.
%
%The current prospective process for modernizing RPG to Java, is tehn represented in Figure \ref{fig:workflowRPG}, where a RPG parser developed in house goes through the RPG code, and post processes this information to resolve data references. This is done with a custom parser due to the nature of RPG code, and its paradigm and structural differences to MDE. From this model based representation of the RPG code, on a immediate phase code generators will produce Java code, wile we develop the ATL rules to abstract the implementation details of RPG into a Platform Independent representation of the data and business logic of the system. Then some of the Synon and RPG code templates are repurposed to convert this higher level of abstraction representation into Java code. This last step will allowing the use of a general code generation that can be used for any project they can convert to this new DSL. At the foreseeable future it will start as Synon and RPG projects.

%Although it is being manually developed, currently the RPG metamodel also inherits from GASTM. as a was to leverage the knowledge acquired during the Synon to Java modernization, leading to a metamodel size as represented in Table \ref{tab:metamodel}. 

%\subsection{RPG modernization project}
%
%After the successful first pilot project, Fresche Legacy saw the efficiency of modernizing legacy applications using MDE.
%They then decided to adapt the process to modernize RPG applications.
%RPG \cite{yaeger1995programming} is a language used to develop programs for AS/400 systems, released in 1959.
%This as lead to a large evolution of the language throughout the years.
%Originaly a procedural language, with strong static typingit, that used a fixed format, so it could be input into the system with use of puched cards, it now allows for free format.
%Many other funcionalities were included, to addapt to more modern requirments.
%The result of this is, when modernizing such systems there is no one pattern of design to follow; the code can be structured to take advantage of reuse or to be delivered with punch cards, it may make use of database access, or be designed for sequencial data, such as tapes.
%
%
%
%\begin{figure*}
%	\centering
%	\includegraphics[width=.7\linewidth, page=2]{images/workflow.pdf}
%	\par
%	\caption{Overview of the process to migrate RPG code to Java \es{we'll revise the figure}}
%	\label{fig:workflowRPG}
%\end{figure*}
%%
%The current prospective process for modernizing RPG to Java, is represented in \Fig{fig:workflowRPG}, where a RPG parser developed in house goes through the RPG code, and post processes this information to resolve data references. This is done with a custom parser due to the nature of RPG code, and its paradigm and structural diferences to MDE. From this model based representation of the RPG code, we use ATL to abstract the implementation details of RPG into a Platform Independent representation of the data and business logic of the system. Then some of the Synon code templates are repurposed to convert this higher level of abstraction representation into Java code. This last step allowing the use of a unified code generation that can be used for both Synon and RPG projects.\vs{update with new info}
%
%Although it is being manualy developed, currently the RPG metamodel also inherits from GASTM. as a was to leverage the knowlage aquired during the Synon to Java modernization, leading to a metamodel size as represented in Table \ref{tab:metamodel}.
%
%
%
%%
%%\begin{table}[h]
%%	\centering
%%	\begin{tabular}{lrr}
%%		\toprule
%%		\textbf{Language} & \textbf{Files} & \textbf{Lines of code}  \\
%%		\midrule
%%		Javascript   & 260 & 99\,879  \\
%%		Java         & 208 & 29\,890  \\
%%		CSS          & 24  & 21\,745  \\
%%		LESS         & 63  & 9\,760   \\
%%		JSON         & 60  & 1\,675   \\
%%		HTML         & 17  & 1\,604   \\
%%		Maven        & 1   & 675    \\
%%		Handlebars   & 15  & 349    \\
%%		SASS         & 1   & 196    \\
%%		DOS Batch    & 1   & 127    \\
%%		Bourne Shell & 2   & 116    \\
%%		XML          & 3   & 91     \\
%%		Python       & 1   & 78     \\
%%		YAML         & 5   & 71     \\
%%		\midrule
%%		Total        & 661 & 166\,256 \\
%%		\bottomrule
%%	\end{tabular}
%%	\caption{Characteristics of the generated application from RPG}
%%	\label{tab:rpg}
%%\end{table}
%
%%\subsection{Scale}
%
%
%%400 hours by hand, an expectation of 40 to 45 hours on automation.
%%1.5 years of process development.
%
%
%%GASTM metamodel
%%193 classes
%%125 references
%%24 attributes

==> feedback.tex <==
\section{Findings} \label{sec:feedback}

\es{Introduce w.r.t. RQs}

In following section we report on the analysis we gathered from the qualitative study.

%From interviewing the staff at Fresche Legacy involved in the usage of MDE to do the migration process we came to the following observations.
% 
%To assess the integration of modeling methodologies and technologies, we conducted some interviews with software engineers involved in the migration process that have integrated modeling into the workflow.
%
%The aim of these interviews is to establish the expectations on modeling technologies, how adjusted are the methodologies to existing workflows.

\subsection{How did the company get into MDE?} \label{sec:discover}

It is interesting to understand how engineers in industry become familiar with a new paradigm.

\subsubsection{Discovery of MDE} \label{sec:discover-mde}

Surprisingly, the initial discovery of MDE was not resulting from contacts with the MDE research community, from conferences, or development forums as generally expected.
Instead, while investigating how competing companies approached the problem of automating the modernization of legacy systems, some reported using the Object Management Group (OMG) standards and practices, which led to further investigation on the subject.
These solutions showed great potential for code generation.
They decided to start using standards and their associated tools to rely on less risky solutions.

However, they felt that compliance to the standards as well as the rigidity of some modeling languages, such as Knowledge Discovery Metamodel (KDM)~\cite{KDM2016} and GASTM, was either too constraining or not  lightweight enough.
Therefore, there was a need to customize the languages in order to facilitate re-engineering of the applications.
MDE showed a broader vision than what they could find directly under the OMG umbrella.
The senior engineer involved in R\&D who discovered about MDE started testing the technology and tools.
This then propagated to other R\&D engineers.

\subsubsection{Self-teaching MDE} \label{sec:learnMDE}

To learn about MDE, domain-specific modeling and associated processes, interviewees reported their main source of knowledge to be tool documentations and forums.
Google searches on software modernization with MDE led to reading the following articles: \cite{Boussaidi2012,7185283,Brunelière20141012,Deltombe2012BridgingKA,Newcomb2010}.
Apart from understanding basic concepts, most learning came from trying and applying small examples in MDE tools.
Their familiarity with programming and traditional software engineering drove this pragmatic way of learning MDE and mostly to see if the technology really worked.
Driven by the tools, they first noted syntactic differences with object-oriented paradigm which then progressed into capturing more subtle difference with the MDE paradigm.

\subsection{How has MDE been integrated in the company?} \label{sec:integrate}

Integrating a new technology, and even more a new paradigm such as MDE, is an important investment for a company that involves risks at the technical level, but also at the social level.

\subsubsection{Natural adaptation to MDE}

Given their extensive software engineering experience, all participants viewed MDE as an extension of their development knowledge with new libraries and associated tools, rather than a new paradigm.
Therefore, they adapted to MDE very pragmatically as if they were acquiring a new programming language.
%
\begin{quote}
	\textit{``I am surprised you ask. Adapting to MDE felt completely natural, just like when I learned Java or Javascript 20 years ago.''} (Interviewee 3)
\end{quote}
%
Modeling is very much anchored with traditional programming and software engineering at Fresche Legacy.

\subsubsection{MDE for automation, not for abstraction}

The primary goal of the projects was to automate the modernization process.
The development strategy started from hand-writing the target application, then iteratively generalize the target application with code templates until it was possible to completely generate the target application.
However, since the hand-coded target application still relied on mimicking the behavior of the legacy application, the logic of the legacy programs remains in the target application.
This resulted in automatically generated Java code that looks like it was implemented by an RPG programmer and not an object-oriented one.
Furthermore, the code generation mimicked closely patterns used by engineers when performing the modernization manually.
Therefore the quality of the generated code, although functionally correct, is difficult to maintain for a Java programmer, given that legacy system concepts and logic are still present.

RPG programmers are very scarce, therefore most hires are Java programmers.
However, they still need to learn Synon and RPG in order to work on modernization projects.
Re-engineering the target application must then remain hand-made.
This task serves to optimize Java code with optimizations that were not possible in the legacy system.
It also serves to support new features like web services and mobile application.
This is why, as stated in \Sect{sec:rpg}, our collaboration promoted the creation of a DSL that abstracts the legacy paradigm and emphasizes on business rules.

We observed that the first models created closely mirrored the structure of the Synon and RPG.
Therefore, most of the complexity in transforming legacy to modern paradigm is encoded in the code generators.
Instead, MDE practitioners would solve this problem using abstraction at the level of models.
Given that the modernization problem involves two very different paradigms (RPG and Java), there is little abstraction concepts in common.
Thus, participants felt compelled to search for a better level of abstraction, that allows independence from the source paradigm, and facilitates the generation of code and re-engineering on the target paradigm.
%
\begin{quote}
	\textit{``I feel it will be easier to generate the code from a DSL than from the abstract syntax tree of RPG.''} (Interviewee 1)
\end{quote}

\es{conclusion: This is one of the main differences where MDE practitioners tend to solve problems as model transformations, whereas non-practitioners tend to rely at the code level.}

\subsubsection{Incrementally integrating MDE}

Given the commercial goals and deadlines of the industry, adoption of MDE had to be restricted at Fresche Legacy.
One reason is because of the time investment needed to learn a new technology that would negatively affect the time needed to be spent on clients projects.
Another reason is because the risk of completely shifting to MDE without a proof of commercial viability is too high.

The first project was a proof of concept on migrating the Synon database that presented more abstractions than RPG using MDE.
Given the complexity of RPG, the company decided to integrate MDE incrementally to mitigate risks.
They started migrating simpler language elements first (\eg \Code{Entities}) and then gradually integrate more complex parts of the language (\eg \Code{Activities}).
This allowed each engineer to invest time on MDE as needed, while being able to continue working on other projects.

Currently, all engineers that were involved (part-time) with the MDE projects are now fully dedicated to further MDE projects.
Therefore the integration of MDE at Fresche Legacy is a success.

\subsection{How did MDE tools help realize the modernization of legacy systems?} \label{sec:tools}

\input{tools}

\subsubsection{Feedback on MDE tools}

The overall feeling regarding the available modeling tools, is that they satisfactorily serve their purpose, but lack maturity.
They provide no significant additional usage facilities, such as accurate and direct feedback from errors, search and comparison functionalities.
This reinforces reinforcing the need for work in line with~\cite{DBLP:conf/models/CuadradoGL15}, where the user is given valuable interactive feedback about transformation errors.
%
\begin{quote}
	\textit{``When you understand how these tools work, it's a lot more flexible [than doing it by hand].''} (Interviewee 2)
\end{quote}

Another issue is the need for a support service behind tools.
They would rather choose a tool that offers support, than investigating for the best tool that lacks support.
For example, they are using EMFText because of the limitations of Xtext, but would prefer to switch to Xtext because of it has a larger user community behind.
Because most of the tools used are part of the Eclipse ecosystem, these projects depend heavily on the Eclipse Modeling Framework (EMF)~\cite{EMF2008}.
This is also felt as a lock-down to the Eclipse platform.
Any MDE tool outside this ecosystem has a much smaller community, but they feel it would be beneficial to have alternatives.
%
\begin{quote}
	\textit{``[...] and sometimes in Eclipse the plugins conflict, so you have to get a different Eclipse installation for each aspect of the project.
		EMF is so bound to eclipse you cannot go to JetBrains or other tools.''} (Interviewee 3)
\end{quote}


\subsection{How does this MDE solution scale to larger modernization projects?} \label{sec:scaleability}

\subsubsection{Environments with performing resources} \label{sec:Dev}

We noted that the development systems used in the company are quite uniform, with an emphasis on large amounts of RAM: around 16 GB.
Depending on the project and the client, production systems may have more resources available.
However, some projects must be run on the client's premises, which may not have high performing resources.
Therefore, the development environment for modernizing of these legacy systems using MDE at full scale is required to have performing resources.
Once the code and process is tested, the migration must still be able to run on less performing resources that clients are restricted to.
Nevertheless, the development environments perform satisfactorily for MDE-based modernization projects.

\subsubsection{Performance is not a problem}

When dealing with such large systems, scalability is usually an issue.
However, in the context of this study, scalability of MDE is not.
The productivity benefits of automatic modernization are orders of magnitude better than manual modernization (see \Sect{sec:success}), that the current state of scalability of MDE is satisfactory enough.
%
\begin{quote}
	\textit{``But of course, any improvement on performance is welcome.''} (Interviewee 1)
\end{quote}

Performance issues have been noted at unexpected points.
For example, this was the case for a transformation with eight ATL rules and three helpers transforming a 3.2 MB Synon model with close to $1.4\times 10^4$ elements into a 89.9 KB model of the DSL with $2.5\times 10^3$ elements.
ATL reported completing the transformation in 500 milliseconds, however the total execution lasted five minutes using 3.5 GB out of 4 GB of RAM with two instances of Eclipse.

%Another case is in tools such as EMFtext where the parsing and verification of the model can take a long time, and in some instances , the model patterns lead into an seamingly infinite parcing loop.
%In this case the behaviour observed whas that the pending tasks in eclipse kept alternating the call of the EMFText parser, and the eclipse verification tools, taking several minutes to reduce the queue of pending processes or in some rare cases keeping the queue at a constant level, ence the conclusion that in those situations if not manualy terminated, the instance of eclipse would remain locked in a loop.

The development team is not worried about the performance of current MDE tools.
They are so used to very large project artifacts that they were used to manage inherent scalability problems even before MDE.
They believe these techniques can transcend to MDE as well.
For example, in this incremental process, they separate larger models into smaller ones in order to make it work in environments with less performing resources.
%
\begin{quote}
	\textit{``[internally] we can generate a subset of the application without having to parse all the files\ldots we can produce a sub-model directly from the Synon tools, which is much easier for me to work with smaller files.''} (Interviewee 3)
\end{quote}

As far as model size is concerned, one would expect the usage of CDO~\cite{CDO} to store and access large models.
Model scale was not a major limiting factor.
They elaborated and adapted a technique using hash maps which was sufficient to increase the performance of (re)loading and searching models.
This was particularly relevant for the model transformation from RPG model to the DSL and for the code generation.

\subsubsection{Robustness of technology}

The only contention point reported was that the MDE-based modernization does not function continuously, unlike in manual modernization.
There is no guarantee of atomicity when running transformations or code generation.
In case of error, we cannot ensure that at least what is produced is correct.
This makes the process quite fragile, in the sense that once it is started it cannot be interrupted or resumed at a later time.
This limits the use of laptops when working on clients premises, where the workstation is restricted to unnecessary up times.
Pause and resume functionalities, recovery points, running as a service, and on-demand execution are desired when executed automated MDE tools, such as model transformation or code generation.


==> metodologies.tex <==
\section{Metodology} \label{sec:Metodologies}

This qualitative case study was performed in order to understand how a company, such as Fresche Legacy, uses MDE technologies without academic expertise influence.
%The boundaries of the case were the experiences of the participants of the two projects 
Although it is a very specific situation, we feel it is rich and unique enough to earn some attention.
%We aimed at discovering the experiences of the subjects, due to the impossibility of performing direct observations and measurements during the course of those projects.

\subsection{Participant selection}\label{sec:participant-selection}

The participants of this study are engineers of the company who have been working with MDE, specifically on either of the two projects presented in \Sect{sec:context}.
This included one senior architect, two on-site developers, and one off-shore developer.
They all account for 12 to 20 years of experience in programming and software engineering.
Their past programming experience was mainly focused on Java development in modernization, framework development, and system emulation.
They have experience with UML modeling, and two of the participants learned UML at the university.
They also reported at some point using CASE tools for requirements extraction and reverse engineering in past modernization projects.

\subsection{Data collection}

We conducted series of informal meetings, semi-structured interviews, and observations.
First, we approached participants with informal conversations and participated as observers in relevant company meetings.
Then, we performed semi-structured interviews to collect answers to our research questions.
Finally, we followed up with informal discussions to clarify some points brought to light during data analysis.
Data retrieved from informal and observational methods was collected during a period of two months.
The formal interviews where held during the last two weeks.
Additionally we collected quantitative data to contextualize our observation and interview data.
This quantitative data came from code inspection reports on the projects, qualification of the modeling and transformation artifacts, and their execution.
We also collected overall data to characterize modernization projects, with information such as project scale and the time manual modernization usually takes for those types of projects.

\subsubsection{Informal meetings}

Informal meetings helped establish contact with the participants and collect background information on the projects.
We also inquired on the use of models and tools to complement our observational data.
These encounters where held in company's office during normal work hours.
Participants were engaged on their free time, or they would engage us to show us specific situations, that then spurred the informal conversation.
The work environment at Fresche Legacy is bilingual, therefore we translated all specific terminology of our notes to English.
At a later stage after the interviews, these informal engagements focused mainly on clarifying or elaborating on responses given during the interview.

\subsubsection{Semi-structured interviews}

The semi-structured interviews where designed in accordance to~\cite{Hove:2005:ECS:1090955.1092163} and~\cite{merriam2015qualitative}.
The interview guideline and questionnaire we followed is available in~\cite{FLFIG2016}.
The authors of~\cite{Hove:2005:ECS:1090955.1092163} recommend that the interviews should focus more on \emph{what} and \emph{how} questions.
However, because we were also interested in the rationale behind the use of MDE technology, we also asked more \emph{why} questions than is usually expected for this type of interview.
Interviews were held during normal work hours, in a closed meeting room ensuring privacy and confidentiality.
They lasted around 30 minutes each.
Only the interviewer and the interviewee were present in the room or via skype for the remote participant.
Unlike the informal meetings, these interviews where held exclusively in English.
Interviewees were free to answer the questions as they saw fit.
All interviews were audio-recorded with the interviewee's consent.
The interviewer then analyzed the recordings and transcribed in writing the most relevant answers of the script.

\subsubsection{Observations}

Observations focused on how engineers use models and MDE tools, relying on observational note taking, inspecting the code, testing ourselves live executions of the modernization process, and taking note of questions raised about MDE or specific tools during internal company meetings.
These observations were performed at the company's office.
We also had access to a laptop provided by their IT department, allowing us to preform the testing by ourselves.

\subsection{Threats to validity}

Like any qualitative study, there are threats to the validity of the study presented here.

We are part of the collaborating effort to further and improve the integration of MDE in the company.
Also data collection took place after we started the collaboration
Therefore, there is a threat to internal validity that there may be some positive bias towards the successful integration of MDE in the company.
We made sure to clarify during the interviews that there were no wrong answers and any criticism to MDE they could pinpoint would be beneficial.
We also crosschecked inconsistencies that came up during our observations to ensure we obtained satisfactory and consistent data.

There are several threats to external validity.
It is difficult to generalize the findings of this study to other companies in the same industry or even other industries in general, due to the specific characteristics of the projects studied.
However, as stated by the participants (see \Sect{sec:discover-mde}) the competition is using MDE, so it is most likely applicable to other companies in the same business domain.
Another threat is the low number of participants interviewed.
We interviewed all of the individuals engaged in MDE at the company, so within this context it was not at all possible to include more individuals.
Hence, we must consider our data as a single data point, in contrast to~\cite{Hutchinson:2011:EAM:1985793.1985858} where many individuals across multiple companies were interviewed.

Finally, there is a threat to the construction of our analysis
We mitigating interpretation errors by collecting quantitative information on the artifacts and processes used, as well as a means to search for inconsistencies in the interviewees answers.
We also followed up with punctual meetings to clarify answers and to make sure we interpreted correctly the data.

